Physics case for an LHCb Upgrade II - Opportunities in flavour physics, and beyond, in the HL-LHC era

The LHCb Upgrade II will fully exploit the flavour-physics opportunities of the HL-LHC, and study additional physics topics that take advantage of the forward acceptance of the LHCb spectrometer. The LHCb Upgrade I will begin operation in 2020. Consolidation will occur, and modest enhancements of the Upgrade I detector will be installed, in Long Shutdown 3 of the LHC (2025) and these are discussed here. The main Upgrade II detector will be installed in long shutdown 4 of the LHC (2030) and will build on the strengths of the current LHCb experiment and the Upgrade I. It will operate at a luminosity up to $ 2 \times 10^{34} \rm cm^{-2}s^{-1}$, ten times that of the Upgrade I detector. New detector components will improve the intrinsic performance of the experiment in certain key areas. An Expression Of Interest proposing Upgrade II was submitted in February 2017. The physics case for the Upgrade II is presented here in more depth. $CP$-violating phases will be measured with precisions unattainable at any other envisaged facility. The experiment will probe $b\to s \ell^+\ell^-$ and $b\to d \ell^+\ell^-$ transitions in both muon and electron decays in modes not accessible at Upgrade I. Minimal flavour violation will be tested with a precision measurement of the ratio of $B(B^0\to\mu^+\mu^-)/B(B_s^0\to \mu^+\mu^-)$. Probing charm $CP$ violation at the $10^{-5}$ level may result in its long sought discovery. Major advances in hadron spectroscopy will be possible, which will be powerful probes of low energy QCD. Upgrade II potentially will have the highest sensitivity of all the LHC experiments on the Higgs to charm-quark couplings. Generically, the new physics mass scale probed, for fixed couplings, will almost double compared with the pre-HL-LHC era; this extended reach for flavour physics is similar to that which would be achieved by the HE-LHC proposal for the energy frontier.

==> CONTRIBUTIONS/7_Rare_and_radiative_decays/7.7.4.tex <==
%\section{Giampi}
\subsection{Search for $\tau \to \mu\mu\mu$ decays}
%Editors: Frederic Teubert \\
%Indicative length: 0.5 pp \\
    \newcommand{\subdecay}[2]{\ensuremath{#1(\!\to #2)}\xspace}
    % Particles
    \def\mupm   {{\ensuremath{\mu^\pm}}\xspace}
    \def\mump   {{\ensuremath{\mu^\mp}}\xspace}
    \def\taupm   {{\ensuremath{\tau^\pm}}\xspace}
    \def\taump   {{\ensuremath{\tau^\mp}}\xspace}
    %% Decays
    \def\taummm{\decay{\taupm}{\mupm \mu^+ \mu^-}}
    \def\Dsetamunu{\decay{\Ds}{\subdecay{\eta}{\mu^+\mu^-\gamma}\mu^+\nu_{\mu}}}
 
 
An important test of the SM is the search for the  lepton-flavour-violating process \taummm. 
Within the SM with zero neutrino masses this process is strictly forbidden. Depending on the mechanism of neutrino mass generation, 
many theories~\cite{Babu:2002et,Brignole:2003iv,Paradisi:2005fk,Hays:2017ekz} beyond the SM predict this branching ratio to be in the region $(10^{-9}-10^{-8})$. 
The current experimental limit~\cite{LHCb-PAPER-2014-052,Hayasaka:2010np,Lees:2010ez}, $\cal{B} (\taummm) <$ $1.2 \times 10^{-8}$, 
is a combination of the results from LHCb and the \bfactories and reaches the starting point of this range. 
\belletwo will probe this interesting region of sensitivity when accumulating up to $50~\rm{ab}^{-1}$. 
The LHC proton collisions at 13 TeV produces $\tau$ leptons, primarily in the decay of heavy flavour hadrons, with a cross-section five orders of magnitude 
larger than at \belletwo. This compensates for the higher background levels and lower integrated luminosity,
and means that during the LHCb \upgradetwo would also be able to probe down to ${\cal O}(10^{-9})$, and independently confirm any \belletwo discovery or 
significantly improve the combined limit. In addition, the proposed improvements to the LHCb calorimeter during the \upgradetwo will be helpful in suppressing 
backgrounds such as \Dsetamunu, enabling LHCb to make best use of its statistical power. 


